Adversarial Masking for Self-Supervised Learning

We propose ADIOS, a masked image model (MIM) framework for self-supervised learning, which simultaneously learns a masking function and an image encoder using an adversarial objective. The image encoder is trained to minimise the distance between representations of the original and that of a masked image. The masking function, conversely, aims at maximising this distance. ADIOS consistently improves on state-of-the-art self-supervised learning (SSL) methods on a variety of tasks and datasets -- including classification on ImageNet100 and STL10, transfer learning on CIFAR10/100, Flowers102 and iNaturalist, as well as robustness evaluated on the backgrounds challenge (Xiao et al., 2021) -- while generating semantically meaningful masks. Unlike modern MIM models such as MAE, BEiT and iBOT, ADIOS does not rely on the image-patch tokenisation construction of Vision Transformers, and can be implemented with convolutional backbones. We further demonstrate that the masks learned by ADIOS are more effective in improving representation learning of SSL methods than masking schemes used in popular MIM models. Code is available at https://github.com/YugeTen/adios.

==> 1introductionv0.tex <==

\section{Introduction} \label{sec:intro}

\begin{wrapfigure}[14]{r}{0.6\textwidth}
    \vspace{-20pt}
    \includegraphics[width=\linewidth]{images/hook-color.png}
    \caption{Mask generated in three different models, namely BERT, Context Encoder \citep{Pathak2016context} and ours.}
    \label{fig:hook}
\end{wrapfigure}

\Acrlong{BERT} \citep{devlin2018bert}, also known as \acrshort{BERT}, is a state-of-the-art method for self-supervised learning in \gls{NLP}.
%
It is a transformer-based model \citep{vaswani2017transformer} trained without supervision to imput missing words in sentences.
%
Specifically, one or more word is removed from an input sentence and replaced with a missing-word token, and the model is asked to predict the whole sentence, including the missing words.

Can the same principle can be applied to image space, and achieve similar booster effect in self-supervised learning?
%
This was first investigated in \citet{Pathak2016context}, where a ``context encoder'' is trained to learn representations by inpainting images that are randomly occluded by fixed-shape masks.
%
While this model achieved competitive results at the time, random masks in pixel space is not equivalent to random word masks in sentences.
%
This is because words are much higher-level representation than pixels, and as a result, contains more structured information than random regions of an image.
%
We visualise this effect in \Cref{fig:hook}: while the words masked out in \gls{BERT} describes a \emph{complete} composition (e.g. head) of the object (first row), the masks used for context encoder often covers only \emph{part} of the feature (second row).
%
The inpainting task for context encoder is therefore a less challenging one, since usually some parts of the entity is available to be used to inpaint the occluded part\footnote{To continue the \acrshort{NLP} analogy, context encoder is perhaps more similar to masking out letters in a sentence.}.

In order to make the inpainting task as challenging as \acrshort{BERT}, we need to generate mask that can occlude complete entities in an image, which requires the mask generation process to utilise the semantic information in images through training.
%
To achieve this, we develop a framework named \textbf{Ad}versarial \textbf{I}npainter-\textbf{O}ccluder \textbf{S}elf-supervision (\acrshort{ADIOS}).
%
As indicated by the name, the model consists of an \emph{inpainter} and an \emph{occluder} that are trained adversarially, with the inpainter imputes missing parts of an image, while the occluder tries to create masks such that inpainting is as difficult as possible.
%
We show the masks generated by the occluder of ADIOS at the bottom row of \Cref{fig:hook}.
%
It is clear that the model does indeed mask out complete components (e.g. head, belly, tail) of the depicted object, creating an imputing task that is similar to BERT's.

The above formulation, albeit intuitive, requires a generative component for inpainting that is redundant for our goal of representation learning. 
%
It has also been discussed in \citet{bao2021beit,ramesh2021zero} that such pixel-level reconstruction tasks waste modelling capacity on high-frequency details instead of low-frequency structure, resulting in subpar performance for representation learning \citep{guangrun, tbpublished}.
%
Inspired by recent advances in self-supervised learning \citep{chen2020simclr, grill2020byol, chen2021simsiam}, we discard the generative component by replacing the inpainter by a Siamese network, which maximises the similarity between the representation of the original image and the occluded image.
%
As per the adversarial learning dynamic, the objective of the occluder is now to create a mask such that the similarity between original vs. occluded image's representations is minimised.
%
We discuss further in \Cref{sec:ae_inpainter} that the Siamese version optimises a functionally similar objective for representation learning to the original generative model, and as we show in \Cref{sec:ea_vs}, results in faster training, better unsupervised learning performance and produces similar quality of masks.

\jimmy{This part will be extended as we perform experiments:}
Benefited from this alteration, our inpainter can adopt any architecture and objective in the Siamese/contrastive self-supervised learning literature, and as we show in empirical evaluation, significantly improve their results on datasets such as ImageNet.
%
Other proposed experiments: 1) compare occluder mask to other unsupervised segmentation methods (object centric) 2) use occluder features/inpainter features for downstream segmentation tasks




==> 1introductionv1.tex <==

\section{Introduction} \label{sec:intro}

\begin{wrapfigure}[14]{r}{0.6\textwidth}
    \vspace{-28pt}
    \includegraphics[width=\linewidth]{images/hook_multiple.png}
    \caption{Masking scheme comparison. \emph{\textbf{BERT}}: mask out words in sentences; \emph{\textbf{Context encoder}}: random, fix-shaped mask; \emph{\textbf{BEiT}}: random ``blockwise'' masking; \emph{\textbf{MAE}}: randomly mask out $75\%$ of the image; \emph{\textbf{Ours}}: multiple masks (N=3) generated by an unsupervised, adversarially trained masking model.}
    \label{fig:hook}
\end{wrapfigure}


\Acrfull{MIM} has attracted a lot of attention in the past few months, pioneering this area are work such as \mae ~\citep{he2021mae} and \beit ~\citep{bao2021beit}.
%
The regime is inspired by the recent advances made in natural language processing by \gls{MLM} such as \bert ~\citep{devlin2018bert}, where the model is trained to impute missing words from context (top row, \Cref{fig:hook}).
%
% This seemingly simple training regime achieved unparalleled performance in self-supervised language modelling.

\mim ~models investigate the following proposal: can the same masking-imputing principle be applied to images, and achieve similar booster effect?
%
This was first investigated in \citet{Pathak2016context}, where a ``context encoder'' is trained to learn representations by imputing images that are randomly occluded by fixed-shape masks.
%
More recently, work such as \mae ~\citep{he2021mae}, \beit ~\citep{bao2021beit} and \ibot ~\citep{zhou2021ibot} propose to adopt a similar regime to infer missing parts of the image occluded by random masks, however they make use of the more powerful \gls{ViT} ~\citep{dosovitskiy2021vit}, which first partitions images into smaller, 16x16 patches, then processes each patch as an ``image token'' -- similar to word tokens in the original transformer.
%
Re-purposing this for \mim ~is then fairly straightforward: randomly masking out an image is equivalent to randomly omitting image tokens as input to the \vit.

While this kind of \mim ~models achieved state-of-the-art results in \acrfull{SSL}, it is important to note that random masks in pixel space is not equivalent to random word masks in sentences.
%
This is because words are much higher-level representation than pixels, and as a result, contains more structured information than random regions of an image.
%
We demonstrate a comparison of these masking schemes in \Cref{fig:hook} to highlight this observation: while the words masked out in \bert ~describes a \emph{complete} composition (e.g. head) of the object (first row), the masks used for context encoder, \beit~ and \mae~ often covers only \emph{part} of the feature (second row, left to right).
%
The imputation task for these models are therefore a less challenging one, since some parts of the entity is often available to be used to infer what's missing\footnote{To continue the \acrshort{NLP} analogy, context encoder is more similar to masking out letters in a sentence.}.

% \jimmy{Not sure whether we single MAE out or not with the following paragraph; in MAE paper they do discuss that the image masks needs to be more challenging to match the BERT masks, and that's why they choose to mask out the majority of the image. but from figure 1 we can see that when masking level is at 75\% (which is what they use during training), it is almost never the case that complete part of the bird/branch is masked out, so I feel like it is also fair to lump them into the same category as BEiT or context encoder.}
% In order to make the inpainting task as challenging as \acrshort{BERT}, we need to generate mask that can occlude complete entities in an image.
% %
% \mae~achieves this by masking out a large proportion of the image (as high as 75\%) (see \Cref{fig:hook}).
% %
% However, we demonstrate through experiments that while this works well for large backbone architecture such as vision transformer, the same masking regime does not seem to be helpful for smaller models, raising question as for whether the model's good representation learning performance rely on memorisation.

In order to make the imputation task in \mim~ comparable to the one in \mlm, we need to generate masks that can occlude complete entities in an image.
 %
To that end, we propose to incorporate semantic information in the mask generation process.
%
We develop a framework named \textbf{Ad}versarial \textbf{I}mputer-\textbf{O}ccluder \textbf{S}elf-supervision (\adios).
%
As indicated by the name, the model consists of an \emph{imputer} and an \emph{occluder} model that are trained adversarially, with the former imputing missing parts of an image, and the latter generating masks such that imputation is difficult.
%
We show the masks generated by the occluder of \adios~at the bottom row of \Cref{fig:hook}.
%
It is clear that the model does indeed mask out complete components (e.g. head, belly, tail) of the depicted object, creating an imputing task that is similar to \bert's.

Conventionally, the inferring of missing information is done in pixel space via inpainting.
%
However, this requires a generative component that is redundant for our goal of representation learning. 
%
It has also been discussed in \citet{bao2021beit,ramesh2021zero} that pixel-level reconstruction tasks waste modelling capacity on high-frequency details instead of low-frequency structure, resulting in subpar performance for representation learning.
%
Both work therefore propose to impute the visual token, instead of raw pixels of the masked input, yielding more efficient, better-performing models.
%
Inspired by these advances, we propose to use an encoder-only imputer: the imputer is now trained to minimise the distance between the \emph{representation} of the original image and the masked image, instead of the distance between their \emph{raw pixel values}.
%
As per the adversarial learning dynamic, the objective of the occluder is to maximise this distance.
%
We discuss further in \Cref{sec:ae_imputer} that the encoder-only imputer optimises a functionally superior objective for representation learning than the generative imputer.
%
Additionally, this Siamese style objective allow us to leverage the recent advances in augmentation-based \acrfull{SSL} \citep{chen2020simclr, grill2020byol, chen2021simsiam} and train our model under different \acrshort{SSL} objectives.
%
We show that ADIOS significantly improves the performance of these \acrshort{SSL} objectives, demonstrating the generalisability of our approach.

% , and as we show in \Cref{sec:ea_vs}, results in faster training, better unsupervised learning performance and produces similar quality of masks.

% \jimmy{This part will be edited as we perform experiments:} 

Our main contribution is a novel, adversarially trained imputer-occluder model for self-supervised learning. 
%
Different from other \mim~methods, our model is not limited to using \vit~as backbone, which is favourable given the recent discoveries on the superiority of modernised ConvNet models over \vit s \citep{2022convnet,touvron2021augmenting}; 
%
additionally, ADIOS can be trained using a range of different \acrshort{SSL} objectives, significantly improving their performance on downstream evaluations including linear probing, unsupervised learning and robustness.
%
We also perform qualitative and quantitative analysis on the masks learned by ADIOS during training, and thoroughly investigate the representation learning performance of models trained with masks generated from different masking schemes, including \mae's $75\%$ mask, \beit's blockwise mask as well as ground-truth object masks.
%
We find models trained with ADIOS and ground-truth masks to significantly outperform other masking schemes/no mask, demonstrating the efficiency of semantically meaningful masks in aiding representation learning. 

==> 1introductionv2.tex <==

\section{Introduction} \label{sec:intro}
%
\begin{wrapfigure}[14]{r}{0.65\textwidth}
    % \vspace{-28pt}
    \vspace{-4em}
    \includegraphics[width=\linewidth]{images/hook_multiple.png}
    \caption{Masking scheme comparison. \emph{\textbf{BERT}}: random word masks; \emph{\textbf{Context encoder}}: random, fix-shaped mask; \emph{\textbf{BEiT}}: random `blockwise' masking; \emph{\textbf{MAE}}: randomly mask out $75\%$ of the image; \emph{\textbf{ADIOS}}: multiple masks (N=3) generated by an adversarially trained masking model.}
    \label{fig:hook}
\end{wrapfigure}
%
\Acrfull{MIM} tries to learn image representations in a self-supervised fashion by occluding parts of the input images.
\Gls{MIM} is inspired by significant advances in natural language modelling such as \bert ~\citep{devlin2018bert}, where the model is trained to fill-in words randomly removed from a sentence (top row, \Cref{fig:hook}).
Indeed, the recent works of \mae ~\citep{he2021mae} and \beit ~\citep{bao2021beit} show that these gains are at least partially transferable to the vision world.
However, unlike in images where small image patches are masked at random, masked tokens in language often correspond to whole entities or relations between them.
In this work, we investigate \emph{learning to mask} motivated by the observation that pixels belonging to a single entity are usually correlated, while pixels belonging to different entities are not.
This allows us to identify and mask out regions of correlated pixels within an image, which brings our method closer to word-masking in natural language; it also results in consistently improved performance of state-of-the-art \gls{SSL} algorithms.

% such as \mae ~\citep{he2021mae} and \beit ~\citep{bao2021beit} have recently produced impressive results 

% \Acrfull{MIM} has attracted a lot of attention in the past few months, pioneering this area are work such as \mae ~\citep{he2021mae} and \beit ~\citep{bao2021beit}.
% %
% The regime is inspired by the recent advances made in natural language processing by \gls{MLM} such as \bert ~\citep{devlin2018bert}, where the model is trained to impute missing words from context (top row, \Cref{fig:hook}).
%
% This seemingly simple training regime achieved unparalleled performance in self-supervised language modelling.

% \mim ~models investigate the following proposal: can the same masking-imputing principle achieve a similar booster effect when applied to images?
%
% This was first investigated in \citet{Pathak2016context}, where a convolutional `context encoder' learns representations by filling-in randomly-occluded image parts.
\Gls{MIM} was first investigated in \citet{Pathak2016context}, where a convolutional `context encoder' learns representations by filling-in randomly-occluded image parts.
%
More recently, this approach has been followed by works such as \mae ~\citep{he2021mae}, \beit ~\citep{bao2021beit} and \ibot ~\citep{zhou2021ibot}.
The masks are still random, but these works use much more powerful \glspl{ViT} ~\citep{dosovitskiy2021vit}, which first partition an image into small patches, then processes each patch as an `image token'---similar to word tokens in the original transformer.
%
Re-purposing this for \mim ~is then fairly straightforward: randomly masking out image parts is equivalent to randomly omitting image tokens as input to the \vit.

While these \mim ~models achieved state-of-the-art results in \acrfull{SSL}, it is important to note that random masks in pixel space are not equivalent to random word masks in sentences.
Words are much higher-level representation than pixels, with a single word's meaning far beyond that of a small randomly-chosen image region.
%
This is highlighted in \Cref{fig:hook}: while the words masked out in \bert ~describes a \emph{complete} composition (e.g. head) of the object (first row), the masks used for context encoder, \beit~and \mae~often cover only a \emph{part} of the feature (second row, left to right).
%
The imputation tasks for these models are therefore less challenging, since some parts of the entity is always visible and can be used to infer the occluded part\footnote{To continue the \acrshort{NLP} analogy, context encoder is more similar to masking out letters in a sentence.}.

% \jimmy{Not sure whether we single MAE out or not with the following paragraph; in MAE paper they do discuss that the image masks needs to be more challenging to match the BERT masks, and that's why they choose to mask out the majority of the image. but from figure 1 we can see that when masking level is at 75\% (which is what they use during training), it is almost never the case that complete part of the bird/branch is masked out, so I feel like it is also fair to lump them into the same category as BEiT or context encoder.}
% In order to make the inpainting task as challenging as \acrshort{BERT}, we need to generate mask that can occlude complete entities in an image.
% %
% \mae~achieves this by masking out a large proportion of the image (as high as 75\%) (see \Cref{fig:hook}).
% %
% However, we demonstrate through experiments that while this works well for large backbone architecture such as vision transformer, the same masking regime does not seem to be helpful for smaller models, raising question as for whether the model's good representation learning performance rely on memorisation.

The comparison between \bert~and models such as \beit~and \mae~in \Cref{fig:hook} suggests that, to make the imputation task in \mim~comparable to the language one, we need to occlude complete entities in an image.
%
\ak{I'm a bit worried about the next sentence; what kind of semantic info are we using?}
To that end, we propose to incorporate semantic information in the mask generation process.
%
We develop a framework named \textbf{Ad}versarial \textbf{I}nference-\textbf{O}cclusion \textbf{S}elf-supervision (\adios).
%
As indicated by the name, the model consists of an inference model and an occlusion model that are trained adversarially, with the former inferring missing parts of an image given the unmasked context, and the latter generating masks such that recovering complete information is difficult.
%
We show the masks generated by \adios~at the bottom row of \Cref{fig:hook} \ak{do we? there is just one mask}.
%
It is clear that the model does indeed mask out complete components (e.g. head, belly, tail) of the depicted object, creating an imputing task that is similar to \bert's.

In general, learning to impute missing information is done by minimising some distance between the original and a corrupted signal.
%
In images, this is conventionally done by minimising a reconstruction loss in the pixel space, e.g., in \citet{Pathak2016context,he2021mae}.
%
However, doing so requires a generative component that is redundant for representation learning. 
%
It has also been discussed in \citet{bao2021beit,ramesh2021zero} that pixel-level reconstruction tasks waste modelling capacity on high-frequency details instead of low-frequency structure, resulting in subpar performance for representation learning.
%
\citet{bao2021beit,ramesh2021zero} therefore propose to impute the visual tokens, instead of pixels of the masked image, yielding more efficient, better-performing models.
%
Inspired by these advances, we propose to train an encoder-only inference model by minimising the distance between the \emph{representation} of the original image and the masked image, instead of the distance between their \emph{raw pixel values}.
%
As per the adversarial learning dynamic \ak{I think very little was said until now about adversarial so as a reader am a bit surprised}, the objective of the occlusion model is to maximise this distance.
\ak{I think we need to give more intuition why this makes sense, i.e., that pixels belonging to an object are correlated while pixels belonging to two different objects or object and background are not correlated, so masks that try to make inpainting harder are likely to cover not necessarily objects but correlated regions in the same---corresponding to words in a sentence}
%
We discuss further in \Cref{sec:ae_imputer} that the encoder-only inference model optimises a functionally superior objective for representation learning than the generative model.
%
Additionally, this Siamese style objective allow us to leverage the recent advances in augmentation-based \acrfull{SSL} \citep{chen2020simclr, grill2020byol, chen2021simsiam} and train our model under different \acrshort{SSL} objectives.
%
We show that ADIOS consistently improves performance of these \acrshort{SSL} objectives, demonstrating generality of our approach.



Our main contribution is a novel, adversarially trained inference-occlusion model for self-supervised learning with the following advantages:
%
\begin{enumerate}
    \item \adios\ can be trained using a range of different \acrshort{SSL} objectives, consistently improving their performance on downstream evaluations including linear probing, unsupervised learning and robustness;
    \item We perform qualitative and quantitative analysis on the masks generated by \adios~ and show that they are semantically meaningful;
    \item Different from other \mim~methods, our model is not limited to using \vit~as backbone, which is favourable given the recent discoveries on the superiority of modernised ConvNet models over \vit s \citep{2022convnet,touvron2021augmenting}; 
    \item We thoroughly investigate representation learning performance of models trained with masks generated from different masking schemes, including masks generated by \adios, \mae's $75\%$ mask, \beit's blockwise mask as well as ground-truth object masks.
    %
    We find models trained with ADIOS and ground-truth masks to significantly outperform other masking schemes/no mask, demonstrating the efficiency of semantically meaningful masks in aiding representation learning. 
\end{enumerate}
%

%

%

%

% Our main contribution is a novel, adversarially trained inference-occlusion model for self-supervised learning. 
% %
% Different from other \mim~methods, our model is not limited to using \vit~as backbone, which is favourable given the recent discoveries on the superiority of modernised ConvNet models over \vit s \citep{2022convnet,touvron2021augmenting}; 
% %
% additionally, ADIOS can be trained using a range of different \acrshort{SSL} objectives, significantly improving their performance on downstream evaluations including linear probing, unsupervised learning and robustness.
% %
% We also perform qualitative and quantitative analysis on the masks learned by ADIOS during training, and thoroughly investigate the representation learning performance of models trained with masks generated from different masking schemes, including \mae's $75\%$ mask, \beit's blockwise mask as well as ground-truth object masks.
% %
% We find models trained with ADIOS and ground-truth masks to significantly outperform other masking schemes/no mask, demonstrating the efficiency of semantically meaningful masks in aiding representation learning. 

==> 1introductionv3.tex <==

\section{Introduction} \label{sec:intro}


% % Concise summary of what MIM is and motivation
% \Acrfull{MIM} tries to learn image representations in a self-supervised fashion by occluding parts of the input images.
% \Gls{MIM} is inspired by significant advances in natural language modelling such as \bert\ \citep{devlin2018bert}, where the model is trained to fill-in words randomly removed from a sentence (top row, \Cref{fig:hook}).
% Indeed, the recent works of \mae\ \citep{he2021mae} and \beit\ \citep{bao2021beit} show that these gains are at least partially transferable to the vision world.
% However, unlike in images where image patches are masked at random (bottom row, \Cref{fig:hook}, masked tokens in language often correspond to whole entities or relations between them (top row).
% % What this work is about
% In this work, we investigate \emph{learning to mask} motivated by the observation that pixels belonging to a single entity are usually correlated, while pixels belonging to different entities are not.
% This results in a novel representation learning algorithm called \textbf{Ad}versarial \textbf{I}nference-\textbf{O}cclusion \textbf{S}elf-supervision (\adios). 
% \adios\ can identify and mask out regions of correlated pixels within an image (bottom right, \Cref{fig:hook})
% which brings it closer to the word-masking regime in natural language; it also results in consistently improved performance of state-of-the-art \gls{SSL} algorithms.

% % What augmentation-based SSL is about.
% % Not sure we need this part here; I put it here because ours is applied to augmentation-based SSL algos so it's a mix of both.
% Augmentation-based \gls{SSL} algorithms for images learn representations that are invariant to perturbations applied to the image---these representations try recover the content of the canonical (unperturbed) image.
% They typically try to minimize the distance in a representation space between two or more \emph{views} of the same image, where each view is created by applying random transformations to that image (e.g., crop, scale, colour jitter).
% To prevent collapse, this mninimization is subject to some constrains, e.g., trying to push representations of dissimilar images apart\footnote{With the notable exception of \cite{chen2021simsiam}, where there is no such constraints and it is unknown why the model does not collapse.}. 

% % What MIM models are about
% \Gls{MIM} models, too, retrieve representation of the canonical (unmasked) image, but to do so, they need to consider correlations between different image parts.
% For example, given an image of a bird in \Cref{fig:hook}, they need to reason about what the bird might be sitting on or what colour the bird's belly is given the visible context (bottom row).
% % MIM vs Bert
% This is similar to \bert\ (top row), but the missing words there describe \emph{complete} entities (e.g. head) of the object. 
% The masks used for context encoder (\cite{Pathak2016context}, which pioneered \gls{MIM}), \beit\ and \mae\ are random, and often cover only an incomplete \emph{part} of an entity (second row, left to right).
% The imputation tasks for these models are therefore less challenging, since some parts of the masked entity is always visible and can be used to infer the occluded part\footnote{To continue the \acrshort{NLP} analogy, context encoder is more similar to masking out letters in a sentence.}.
% Consequently, \cite{he2021mae} observed masking large fractions of the image is essential for good performance.
% In contrast, the comparison with \bert\ in \Cref{fig:hook} as well as our results (bottom row, right) suggests that what is masked may be at least as important as how much is masked.

% Concise summary of what MIM is and motivation
\Acrfull{MIM} tries to learn image representations in a self-supervised fashion by occluding parts of the input images.
\Gls{MIM} is inspired by significant advances in natural language modelling such as \bert\ \citep{devlin2018bert}, where the model is trained to fill-in words randomly removed from a sentence (\Cref{fig:hook}, top row).
Indeed, the recent works of \mae\ \citep{he2021mae} and \beit\ \citep{bao2021beit} show that these gains are at least partially transferable to vision.
% MIM vs Bert
The task of a \gls{MIM} model is therefore similar to \bert, e.g., given an image of a bird in \Cref{fig:hook}, it needs to reason about what the bird might be sitting on or what colour the bird's belly is given the visible context (bottom row).
%
However, while missing words describe \emph{complete} entities (e.g. head), the masks used for context encoder (\citet{Pathak2016context}, which pioneered \gls{MIM}), \beit\ and \mae\ are random, and therefore often cover only an incomplete \emph{part} of an entity (second row, left to right).
%
As a result, the imputation tasks for these models are less challenging, since some parts of the masked entity is always visible and can be used to infer the occluded part\footnote{To continue the \acrshort{NLP} analogy, context encoder is more similar to masking out letters in a sentence.}.
%
Consequently, \citet{he2021mae} observed that masking large fractions of the image is essential for good performance.
%
In contrast, the comparison with \bert\ in \Cref{fig:hook} (bottom row, right) as well as our empirical results suggests that \emph{what is masked} may be at least as important as \emph{how much is masked}.


\begin{figure}[t]
    \includegraphics[width=\linewidth]{images/hook_multiple.png}
    \caption{
        % Masking scheme comparison.
        Self-supervised language and vision models can learn by imputing data removed by masking.
        \emph{\textbf{BERT}}: random word masks; \emph{\textbf{Context encoder}}: random, fix-shaped mask; \emph{\textbf{BEiT}}: random `blockwise' masking; \emph{\textbf{MAE}}: randomly mask out $75\%$ of the image; \emph{\textbf{ADIOS}}: multiple masks (N=3) generated by an adversarially trained masking model, post-processed with fully connected conditional random fields \citep{crf}.
    }
    \label{fig:hook}
\end{figure}


% What this work is about
It is instructive to note that, usually, pixels belonging to a single entity are strongly correlated, while pixels belonging to different entities are not.
Therefore, masking a whole entity removes all strongly-correlated pixels, making it much more difficult to reason about the missing region---now it is only possible by considering relations with the rest of the image.
% Any model that solves this task has to reason about relations between different entities.
Therefore, in effort to make the vision setting more similar to \bert, we investigate \emph{learning to mask} with an adversarial objective, where an \emph{occlusion model} is asked to make reasoning about missing parts of the scene more difficult. 
This results in a novel representation learning algorithm called \textbf{Ad}versarial \textbf{I}nference-\textbf{O}cclusion \textbf{S}elf-supervision (\adios). 
\adios\ can identify and mask out regions of correlated pixels within an image (\Cref{fig:hook}, bottom right)
which brings it closer to the word-masking regime in natural language; it also results in consistently improved performance of state-of-the-art \gls{SSL} algorithms.

Note that the existing \gls{MIM} models are trained by reconstructing the masked image. 
Since this requires a redundant generative component, we frame \adios\ as an encoder-only framework that minimises the distance between the \emph{representation} of the original image and the masked image.
% This enables pairing \adios\ with different Siamese \gls{SSL} algorithms.
Additionally, we have an occlusion model that is trained adversarially: it tries to maximise that distance.
We further discuss in \Cref{sec:ae_imputer} that, compared to the generative setup, the encoder-only setup optimises a functionally superior objective for representation learning.
%
Note that the encoder objective is compatible with many recent augmentation-based Siamese \acrfull{SSL} \citep{chen2020simclr, grill2020byol, chen2021simsiam} methods.
%
We show that \adios\ consistently improves performance upon these \acrshort{SSL} objectives, demonstrating generality of our approach.

Our main contribution are are follows,
%
\begin{enumerate}[topsep=-0.5em,itemsep=0em,partopsep=0em,parsep=0em,leftmargin=*]
    \item A novel adversarial Siamese-style \gls{MIM} framework.
    Unlike other \mim\ methods, ours is not limited to using \vit\ as a backbone, which is favourable given the recent discoveries on the superiority of modernised convnets over \vit s \citep{2022convnet,touvron2021augmenting}; 
    % 
    \item A qualitative and quantitative analysis showing that the masks generated by \adios\ are semantically meaningful;
    \item An analysis of how different masking schemes affect representation learning performance of \gls{SSL} models.
    %
    We find that models trained with ADIOS and ground-truth masks to significantly outperform other masking schemes/no mask, demonstrating the efficiency of semantically meaningful masks in aiding representation learning. 
\end{enumerate}

% % how MIM models rely on tokenization; this might be more relevant for rel works than intro
% \Gls{MIM} was first investigated in \citet{Pathak2016context}, where a convolutional `context encoder' learns representations by filling-in randomly-occluded image parts.
% More recently, this approach has been followed by works such as \mae\ \citep{he2021mae}, \beit\ \citep{bao2021beit} and \ibot\ \citep{zhou2021ibot}.
% The masks are still random, but these works use much more powerful \glspl{ViT}\ \citep{dosovitskiy2021vit}, which first partition an image into small patches, then processes each patch as an `image token'---similar to word tokens in the original transformer.
% Re-purposing this for \mim\ is then fairly straightforward: randomly masking out image parts is equivalent to randomly omitting image tokens as input to the \vit.

% % What augmentation-based SSL is about.
% % Not sure we need this part here; I put it here because ours is applied to augmentation-based SSL algos so it's a mix of both.
% Augmentation-based \gls{SSL} algorithms for images learn representations that are invariant to perturbations applied to the image---these representations try recover the content of the canonical (unperturbed) image.
% They typically try to minimize the distance in a representation space between two or more \emph{views} of the same image, where each view is created by applying random transformations to that image (e.g., crop, scale, colour jitter).
% To prevent collapse, this mninimization is subject to some constrains, e.g., trying to push representations of dissimilar images apart\footnote{With the notable exception of \cite{chen2021simsiam}, where there is no such constraints and it is unknown why the model does not collapse.}. 


% % Move this to method/discussion/related work
% \Gls{MIM} models are trained by minimising reconstruction error with respect to the original image \citet{Pathak2016context,he2021mae}.
% However, if representation learning is the goal, this requires a redundant generative component.
% Additionally, pixel-level reconstruction may spend modelling capacity on high-frequency details instead of low-frequency structure, resulting in subpar performance for representation learning \citet{bao2021beit,ramesh2021zero}.
% %
% We therefore propose to train 
% \ak{it'd be good to further connect it with SSL}

==> 2methods.tex <==
\section{Methodology}

\begin{wrapfigure}[10]{r}{0.3\textwidth}
    \vspace{-20pt}
    \includegraphics[width=\linewidth]{images/model.pdf}
    \vspace{-10pt}
    \caption{\gls{ADIOS} architecture.} % The occluder first produce a mask $m$ from the image $x$, which is then applied to the image via element-wise product $x\cdotm$. The inpainter extracts features $z$ and $\tilde{z}$ from the original image $x$ and the occluded image $x\cdotm$ respectively. The inpainter and the occluder play a min-max game, where the inpainter is trained to maximise the similarity between $z$ and $\tilde{z}$ and the occluder minimises it.}
    \label{fig:architecture}
\end{wrapfigure}

Our framework \gls{ADIOS} consists of two componenets, an inpainter $\Itheta$ and an occluder $\Mpsi$ (see \Cref{fig:architecture}). 
%
Given an RGB image $x \in \RR^{h \times w \times c}$, the occluder produces a binary mask $\Psi:x\mapsto m$, where $m \in \{0, 1\}^{h \times w}$.
%
The inpainter $\Itheta$ takes the original image $x$ and the occluded image $x_m = x\odot m$ as input, and extracts representations $z=\Itheta(x)$ and $z_m=\Itheta(x_m)$ for both images.
%
Parameters of inpainter and occluder $\Theta$ and $\Psi$ are learned by solving the following min-max problem
%
\begin{align}
    \Theta^\star, \Psi^\star = \arg\max_\Theta\min_\Psi \mathcal{D}(z,z_m), \label{eq:minmax_obj}
\end{align}
%
where $\mathcal{D}$ is some distance metric defined in $\RR^d$.
We will now introduce each component in details.

\subsection{Inpainter $\Theta$} 
%
\paragraph{Generative inpainter} Our original motivation for the inpainter $\Theta$ is clear from its name: the inpainter should take an masked image. i.e. $x\odot m$, and \emph{inpaint} the missing part to recover the original image $x$.
%
For clarify purposes, we refer to this version of inpainter as the generative inpainter.

While there are many options to address the inpainting problem, since our goal is to learn useful representations, we limit our discussion to latent-variable models, specifically \gls{VAE}s.
%
We propose to adopt the \gls{VAEAC} model \citep{ivanov2019vaecondarb} as our generative inpainter, which has been successfully applied to image inpainting tasks.
%
\gls{VAEAC} approximates the conditional distribution of the unobserved part of the image $\bar{x}_m=x\odot(1-m)$ given the observed image $x_m$ and the mask $m$, via the following \gls{ELBO}
%
\begin{align}
    \mathcal{L}(x,m;\phi,\theta,\psi) = \EE_{\q{z}{x,m}{\phi}}{\log\frac{\p{\bar{x}_m}{z,x_m,m}{\theta}\p{z}{x_m, m}{\psi}}{\q{z}{x,m}{\phi}}} \leq \log  p(\bar{x}_m | x_m, m) \, ,\label{eq:vaeac_obj}
    % \log &\ p(\bar{x}_m | x_m, m)\notag \\
    % &\geq \EE_{\q{z}{x,m}{\phi}}{\log\p{\bar{x}_m}{z,x_m,m}{\theta}} - \KL{\q{z}{x,m}{\phi}}{\p{z}{x_m, m}{\psi}} = \mathcal{L}(x,m;\phi,\theta,\psi)\, ,
\end{align}
%
where $\q_\phi$ denotes the inference network, $\p_\psi$ the prior network and $p_\theta$ the generative model.
%
These three components form our generative inpainter, where $\Theta = \{\phi, \psi, \theta\}$.

\paragraph{Discriminative inpainter} 
%
Since our goal here is representation learning, the generative component $\theta$ in our inpainter is redundant.
%
To derive a useful objective without the generative model, let us consider learning only the encoding network for the partially-observed image, i.e. the prior network $p_\psi$, under the objective in \Cref{eq:vaeac_obj}.
%
We can write the gradient with respect to $\psi$ as
%
\begin{align}
    \nabla_{\psi}\mathcal{L}(x,m;\phi,\theta,\psi) = \nabla_{\psi} \KL{\q{z}{x,m}{\phi}}{\p{z}{x_m, m}{\psi}}.
\end{align}
%
When considering the learning of $\psi$ independently, the objective in \Cref{eq:vaeac_obj} reduces to minimising the KL divergence between the encoding distribution of $x$ and $x_m$.
%
This is crucial for the task of inpainting, since during training, the generative model only has access to the latent sampled from the encoding distribution of the full image --
%
in order to perform inpainting well at test time, the samples from the encoding distribution of the partially observed image $p_\psi(\cdot)$ should be as similar as possible to that of the full image $q_\phi(\cdot)$.

Following this principle, we can simply learn the encoding networks $\phi$ and $\psi$ under a discriminative model setting.
%
We can further relax the objective by specifying that $q_\phi(\cdot)$ and $p_\psi(\cdot)$ need not be distributions, and simply performs mapping $\phi: x \mapsto m$ and $\psi: x_m \mapsto z_m$.
%
This allows us to replace the KL by some distance metric $\mathcal{D}$.
%
Our new discriminative objective therefore becomes
%
\begin{align}
    \mathcal{L}(x,m; \phi,\psi) = \mathcal{D}(q_\phi(x), p_\psi(x_m)) = \mathcal{D}(z, z_m)\,.
\end{align}




==> 2methodsv1.tex <==
\section{Methodology}

\begin{wrapfigure}[8]{r}{0.35\textwidth}
    \vspace{-30pt}
    \includegraphics[width=\linewidth]{images/model_ambiguous.pdf}
    \vspace{-10pt}
    \caption{ADIOS Architecture.} % The occluder first produce a mask $m$ from the image $x$, which is then applied to the image via element-wise product $x\cdotm$. The inpainter extracts features $z$ and $\tilde{z}$ from the original image $x$ and the occluded image $x\cdotm$ respectively. The inpainter and the occluder play a min-max game, where the inpainter is trained to maximise the similarity between $z$ and $\tilde{z}$ and the occluder minimises it.}
    \label{fig:architecture}
\end{wrapfigure}

\paragraph{Set up} Our framework ADIOS consists of two componenets, an inpainter $\Itheta$ and an occluder $\Mpsi$ (see \Cref{fig:architecture}). 
%
Given an RGB image $\x$, the occluder produces a binary mask $\m=\Mpsi(\x)$, where $\m \in \{0, 1\}^{h \times w}$ and $\x \in \RR^{c \times h \times w}$.
%
The inpainter $\Itheta$ takes the original image $\x$ and the occluded image $\x^{\m} = \x\odot \m$ as input and computes a loss $\mathcal{L}_{\text{ADIOS}}$.
%
Parameters of inpainter  $\Theta$ and occluder $\Psi$ are learned by solving the following min-max problem
%
\begin{align}
    \Theta^\star, \Psi^\star = \arg\min_\Theta\max_\Psi \mathcal{L}_{\text{ADIOS}}(\x;\Theta, \Psi) . \label{eq:minmax_obj}
\end{align}
%
We will now introduce each component in details.

\subsection{Inpainter $\Itheta$}
%
In this section we discuss a few different forms of inpainter and develop their respective objective $\mathcal{L}$ that can be used to optimise \Cref{eq:minmax_obj}.
%
We show how we arrive at our final objective with augmentation based \acrfull{SSL} methods as backbone and discuss its benefits.
%
\paragraph{Auto-encoding Inpainter} \label{sec:ae_inpainter}
%
In \citet{Pathak2016context}, authors proposed context encoder that learns image representations without supervision by inpainting images that are randomly occluded.
%
They define their inpainter $\Itheta$ as an auto-encoder consisting of encoder $q_\phi$ and decoder $p_\theta$, such that $\mathcal{I}_{\Theta} = p_\theta \circ q_\phi$.
%
The model is trained using the following reconstruction loss
%
\begin{align}
    \mathcal{L}_{\text{rec}}(\x; \Theta, \Psi) = \mathcal{D}(\x, p_\theta \circ q_\phi (\x\odot \m)) = \mathcal{D}(\x, \Itheta (\x^{\m})), \label{eq:inpainter_ae_obj}
\end{align}
%
where $\m = M_\Psi(\x)$ and $\mathcal{D}$ denotes some distance metric defined in the image space\footnote{Original paper uses L2. Also, in the original paper $\mathcal{L}_{\text{rec}}$ is computed only for the masked out region, which we omit here for simplicity.}.
%
Minimising this loss encourages the the autoencoder to inpaint the missing part of the image as accurately as possible. 
%
We can plug $\mathcal{L}_{\text{rec}}$ in \Cref{eq:minmax_obj} as $\mathcal{L}_{\text{ADIOS}}$ in and use it to train the inpainter-occluder model.

\paragraph{Encoding Inpainter}
%
An interesting question to ask about the auto-encoding inpainter is: where does the inpainting happen in the model? 
%
There are a few possible hypotheses: 
%
\circled{1} \emph{\textbf{Encoder only:}} The encoder $q_\phi$ completely recovers the missing information in $\x^{\m}$, such that $q_\phi(\x^{\m}) = q_\phi(\x)$; the decoder reconstructs the representations learned from the encoder faithfully.
%
\circled{2} \emph{\textbf{Decoder only:}} The encoder faithfully extracts all information from $\x^{\m}$, and the decoder reasons to inpaint missing pixel from the representations;
%
\circled{3} \emph{\textbf{Both:}} The encoder and decoder both inpaints part of the image.

While three scenarios are all possible, \circled{1} is undoubtedly the most powerful for representation learning, as it requires the the encoder to not only extract features from the observed image, but also reason for the missing part based on the observed context.
%
Since representation learning (instead of image inpainting) is our eventual goal --- is it possible to design an objective targetting scenario \circled{1} such that we learn the most expressive version of $q_\phi$?

One key observation of \circled{1} is that when the encoder recovers all information of the image, $q_\phi(\x^{\m}) = q_\phi(\x)$, that is, the feature extracted from the partially observed image $\x^{\m}$ is the same as the full image $\x$.
%
We therefore propose an encoding inpainter $\Itheta$, which consists of only the encoder and extracts representation from image via $\z =\Itheta(\x)$, where $\z\in\RR^d$.
%
Our objective can therefore be written as 
%
\begin{align}
    \mathcal{L}_{\text{enc}}(\x;\Theta,\Psi) = \mathcal{D}(\Itheta(\x), \Itheta(\x\odot \m))=\mathcal{D}(\z,\z^{\m}), \label{eq:inpainter_siamese_obj}
\end{align}
%
where $\mathcal{D}$ is some distance metric defined in $\RR^d$.
%
Not only does $\loss_{\text{enc}}$ encourages the learning of more expressive encoder that can perform inpainting, optimising this objective also does not involve generative component $p_\theta$, which is redundant for representation learning.


% \begin{wrapfigure}[13]{r}{0.45\textwidth}
% \vspace{-20pt}
% \begin{minipage}{0.49\linewidth}
%     \centering\captionsetup[figure]{justification=centering}
%     \includegraphics[width=\linewidth]{images/simclr.pdf}
%     \vspace{-20pt}
%     \caption{SimCLR.}\label{fig:5a}
% \end{minipage}
% \hfill
% \begin{minipage}{0.49\linewidth}
%     \centering\captionsetup[figure]{justification=centering}
%     \includegraphics[width=\linewidth]{images/simclr_inpainter.pdf}
%     \vspace{-15pt}
%     \caption{SimCLR inpainter.}\label{fig:5a}
% \end{minipage}
% \end{wrapfigure}
\begin{wrapfigure}[9]{r}{0.32\textwidth}
\vspace{-25pt}
\includegraphics[width=\linewidth]{images/simclr+inpainter_c.png}
\vspace{-10pt}
\caption{\textbf{\emph{Left}}: SimCLR. \textbf{\emph{Right}}: SimCLR adapted for ADIOS. }\label{fig:simclr+inpainter}
\end{wrapfigure}

\paragraph{\acrshort{SSL} inpainter} 
%
\Cref{eq:inpainter_siamese_obj} can be realised by simply optimising a Siamese network \citep{bromley1993siamese}.
%
However, this loss can be trivially minimised when all the representations for different inputs ``collapse'' to a constant.
%
This phenomenon is known as latent collapse, and has been addressed in many different ways in augmentation-based \acrshort{SSL}.
% where similar to \cref{eq:inpainter_siamese_obj}, the goal is to minimise the distance between the representations of two augmented views of the same image.
%
% For instance, SimCLR \citep{chen2020simclr} utilises minibatch training, and repulses the representation of different images while attracting the same image's two augmented views; BYOL \citep{grill2020byol} prevents collapse by using a momentum encoder; SimSiam \citep{chen2021simsiam} does so by implementing a stop gradient operation for one of the Siamese network's forward pass.
%
% Notably, despite their differences, almost all augmentation-based \acrshort{SSL} methods optimise a loss that involves the term in \Cref{eq:inpainter_siamese_obj}. 

To understand how this is relevant to our model, let us take SimCLR \citep{chen2020simclr} as an example (see \Cref{fig:simclr+inpainter}, left); given a minibatch of $N$ input images $\x =\{\x_i\}_{i=1}^{N}$, two sets of random augmentations $A$ and $B$ are applied to each image in $\x$, yielding $\x^A$ and $\x^B$. 
%
Both sets of augmented views are passed through the same encoding function, which we simplify as $f_\Theta$, to acquire the representation $\z^A=f_\Theta(\x^A)$ and $\z^B=f_\Theta(\x^B)$.
%
The objective of SimCLR is defined as
%
\begin{align}
%\{\x^A_i, \x^B_i\}_{i=0}^N
    \mathcal{L}_{\text{SimCLR}}(\x; \Theta) = \log \frac{\exp(\mathcal{D}(\z^A_i, \z^B_i)/\tau)}{\sum^{2N}_{j=1} \mathbbm{1}_{[i\neq j]}(\exp(\mathcal{D}(\z^A_i, \z^B_j))/\tau)}, \label{eq:simclr_obj}
\end{align}
%
where $\mathcal{D}(\u, \v)=-\u^T\v / \left\| \u \right\| \left\| \v \right\|$ denotes the negative cosine similarity between $\u$ and $\v$, $\mathbbm{1}_{[i\neq j]}\in \{0,1\}$ is an indicator function that gets the value 1 if $i\neq j$ and 0 otherwise, and $\tau$ denotes a temperature parameter.
%
Intuitively, the objective minimises the distance between representations of the two augmented views of the same image (i.e. $\z^A_i, \z^B_i$), while repulsing the representations of different images (i.e. $\z^A_i, \z^B_j$).
%
This effectively prevents the representations of different images from collapsing to the same constant, while optimising an objective similar to \Cref{eq:inpainter_siamese_obj}.
% For instance, SimCLR \citep{chen2020simclr} utilises minibatch training, and repulses the representation of different images while attracting the same image's two augmented views; BYOL \citep{grill2020byol} prevents collapse by using a momentum encoder; SimSiam \citep{chen2021simsiam} does so by implementing a stop gradient operation for one of the Siamese network's forward pass.
%

W can use the SimCLR objective for our model by applying mask to one of the augmented image and then follow the exact same pipeline (see \Cref{fig:simclr+inpainter}, right).
%
More specifically, we replace $x^A$ by $\x^{A,m}=\x^A\odot \m^A$, where $\m^A = \Mpsi(\x^A)$ is a mask generated by the occluder given $\x^A$ as input.
%
Following \Cref{eq:simclr_obj}, we can write the SimCLR-ADIOS objective as
%
\begin{align}
    \mathcal{L}_{\text{SimCLR\_ADIOS}}(\x; \Theta, \Psi) = \log \frac{\exp(\mathcal{D}(\z^{A,m}_i, \z^B_i)/\tau)}{\sum^{2N}_{j=1} \mathbbm{1}_{[i\neq j]}(\exp(\mathcal{D}(\z^{A,m}_i, \z^B_j))/\tau)}\, . \label{eq:simclr_adios_obj}
\end{align}
%
Again, we can use $\mathcal{L}_{\text{SimCLR\_ADIOS}}$ in \Cref{eq:minmax_obj} to train the occluder and the  inpainter.
%
Importantly, any \acrshort{SSL} method that compares the two augmented views of an image includes a term like \Cref{eq:inpainter_siamese_obj} and can be plugged in to our framework.
%
We conducted experiments using the objective of SimCLR, BYOL \citep{grill2020byol} and SimSiam \citep{chen2021simsiam}, and show improvement on downstream task performance of each method significantly.

\subsection{Occluder $\Mpsi$}
%
For the sake of simplicity, we only considered the case where the occluder produces one mask only in the discussion above.
%
In reality, since an image usually contains multiple components, we generate $K>1$ masks with the occluder to challenge the model to inpaint different components, which we find in experiments is more beneficial for representation learning.

There are many parametric forms of $\Psi$ we could employ --- for instance, one could consider generating multiple masks sequentially in an auto-regressive manner as seen in \citet{engelcke2021genesis}.
%
However, here we find that the simplest solution suffice, where $\Psi: \RR^{c \times w \times h} \mapsto \RR^{K \times w \times h}$ consists of a learnable neural network $f_\psi$, and a softmax layer $\sigma$ applied across $K$ masks to ensure that all the masks sums to 1.
%
We have also experimented with binarising the masks during training and use a straight-through estimator for computing gradients\footnote{In PyTorch this can be implemented as \texttt{mask = binary\_mask + (mask - binary\_mask).detach()}.}, however we find that this does not improve results and therefore used real-valued masks directly.


\subsection{Putting it together}

\begin{wrapfigure}[8]{r}{0.4\textwidth}
    \vspace{-30pt}
    \includegraphics[width=\linewidth]{images/model_ambiguous_k.pdf}
    \vspace{-10pt}
    \caption{ADIOS architecture (K>1).} % The occluder first produce a mask $m$ from the image $x$, which is then applied to the image via element-wise product $x\cdotm$. The inpainter extracts features $z$ and $\tilde{z}$ from the original image $x$ and the occluded image $x\cdotm$ respectively. The inpainter and the occluder play a min-max game, where the inpainter is trained to maximise the similarity between $z$ and $\tilde{z}$ and the occluder minimises it.}
    \label{fig:architecture_k}
\end{wrapfigure}

Here we present the final form of ADIOS incorporating the $K$-masks occluder.
%
The occluder first produces $K$ soft masks $\{\m_i\}_{i=1}^K$ from the RGB image $\x$. 
%
The inpainter computes a loss $\mathcal{L}(\x,\m_i;\Theta)$ for each $\m_i$ and the final loss is computed by averaging across $K$ masks
%
\begin{align}
    \mathcal{L}_{\text{ADIOS}}(\x;\Theta, \Psi) = \frac{1}{K} \sum^K_{i=1} \mathcal{L}(\x,\m_i;\Theta).
\end{align}
%
This objective can be plugged in to \Cref{eq:minmax_obj} to optimise both the inpainter and the occluder in an adversarial manner. 
%
We also include the pseudocode of ADIOS in \Cref{alg:adios}.


\begin{center}
\scalebox{0.9}{
\begin{minipage}[t]{0.7\linewidth}
\begin{algorithm}[H]
\SetAlgoNoLine
    \Function{ADIOS(xA, xB, inpainter, occluder):}{
    \ masks = occluder(xA) \Comment{generate masks}
    \ loss = [] \;
    \For{\KwFor mask \KwIn masks:}{
        \ xAm = xA * mask \\
        \ loss.append(inpainter(xAm, xB))
        }
    \ \Return sum(loss)/len(loss)
    } 
    \;
    \Comment{main training loop}
    \For{\KwFor x \KwIn loader:}{
        \ xA, xB = aug(x), aug(x) \Comment{random augmentation}
        \Comment{forward pass, inpainter}
        \ loss\_i = ADIOS(xA, xB, inpainter, occluder) \;
        \ loss\_i.backwards() \;
        \ update(inpainter) \;
        \Comment{forward pass, occluder}
        \ loss\_o = -ADIOS(xA, xB, inpainter, occluder) \;
        \ loss\_o.backwards() \;
        \ update(occluder) \;
    }

\caption{Pseudocode (PyTorch-style) for ADIOS.}
\label{alg:adios}
\end{algorithm}
\end{minipage}}
\end{center}


==> 2methodsv2.tex <==
\section{Methodology}
%
\begin{wrapfigure}[8]{r}{0.5\linewidth}
    \vspace{-20pt}
    % \vspace{-2em}
    \includegraphics[width=\linewidth]{images/model_ambiguous.png}
    \vspace{-10pt}
    \caption{ADIOS Architecture.} % The occluder first produce a mask $m$ from the image $x$, which is then applied to the image via element-wise product $x\cdotm$. The imputer extracts features $z$ and $\tilde{z}$ from the original image $x$ and the occluded image $x\cdotm$ respectively. The imputer and the occluder play a min-max game, where the imputer is trained to maximise the similarity between $z$ and $\tilde{z}$ and the occluder minimises it.}
    \label{fig:architecture}
\end{wrapfigure}
%
\paragraph{Set up} 
Our framework ADIOS consists of two componenets, an inference model $\I$ and an occlusion model $\M$ (see \Cref{fig:architecture}). 
%
Given an RGB image $\x$, the occlusion model produces a binary mask $\m=\M(\x)$.
% , where $\m \in \{0, 1\}^{h \times w}$ and $\x \in \RR^{c \times h \times w}$
The inference $\I$ takes the original image $\x$ and the occluded image $\x^{\m} = \x\odot \m$ as input and computes a loss $\mathcal{L}$, where $\odot$ denotes the hadamard product.
%
The two models are learned by solving the following min-max problem
%
\begin{align}
    \I^\star, \M^\star = \arg\min_\I\max_\M \mathcal{L}(\x; \I, \M) . \label{eq:minmax_obj}
\end{align}
%
We will now introduce each component in details.

\subsection{Inference model $\I$}
%
As discussed in \Cref{sec:intro}, the inference model should minimise some distance between the original and the masked image.
%
In this section, we discuss a few different instantiation of this objective, and eventually arriving at our final framework using augmentation-based \acrfull{SSL} methods.
%
\paragraph{Distance in pixel space} \label{sec:ae_imputer}
%
One straightforward realisation to the proposed objective is to use the inference model to inpaint the masked image, and train $\I$ by minimising the distance between the inpainted image and the original image in pixel space.
%
More specifically, $\I$ is parametrised by an auto-encoder consisting of encoder $q$ and decoder $p$. 
%
The model can be trained using the following reconstruction loss
%
\begin{align}
    \mathcal{L}_{\text{AE}}(\x; \I, \M) &= \mathcal{D}(\x, p \circ q (\x^{\m}))\notag \\
    &= \mathcal{D}(\x, \I (\x\odot \M(\x))), \label{eq:imputer_ae_obj}
\end{align}
% = 
where $\mathcal{D}$ denotes some distance metric defined in the pixel space.
%
Minimising this loss encourages the the auto-encoder to impute the missing part of the image as accurately as possible. 
%
$\mathcal{L}_{\text{AE}}$ can be used in \Cref{eq:minmax_obj} to train the inference-occlusion model.

\paragraph{Distance in representation space}
%
An interesting question to ask about the auto-encoding $\I$ is: where does the imputation happen in the model? 
%
There are several possible hypotheses: 
%
\circled{1} \emph{\textbf{Encoder only:}} The encoder $q$ completely recovers the missing information in the masked image, such that $q(\M(\x)) = q(\x)$; the decoder reconstructs the representations learned from the encoder faithfully.
%
\circled{2} \emph{\textbf{Decoder only:}} The encoder faithfully extracts all information from the masked image, and the decoder reasons to inpaint missing pixel from the representations;
%
\circled{3} \emph{\textbf{Both:}} The encoder and decoder both inpaints part of the image.

While three scenarios are all possible, \circled{1} is undoubtedly the most powerful for representation learning, as it requires the the encoder to not only extract features from the observed image, but also reason for the missing part based on the observed context.
%
Since representation learning (instead of image inpainting) is our eventual goal --- is it possible to design an objective targetting scenario \circled{1} such that we learn the most expressive version of $q$?

One key observation of \circled{1} is that when the encoder recovers all information of the image, $q(\x^{\m}) = q(\x)$, that is, the feature extracted from the partially observed image $\x^{\m}$ is the same as the full image $\x$.
%
We therefore propose an encoding inference model $\I$, which consists of only the encoder and extracts representation from image via $\z =\I(\x)$, where $\z\in\RR^d$.
%
Our objective can therefore be written as 
%
\begin{align}
    \mathcal{L}_{\text{ENC}}(\x;\I, \M) &=\mathcal{D}(\z,\z^{\m}) \notag \\
     &= \mathcal{D}(\I(\x), \I(\x\odot \M(\x))),
    \label{eq:imputer_siamese_obj}
\end{align}
%
where $\mathcal{D}$ is some distance metric defined in $\RR^d$.
%
Not only does $\loss_{\text{ENC}}$ encourages the learning of more expressive encoder that can infer missing information, optimising this objective also does not involve generative component $p$, which is redundant for representation learning.


\begin{wrapfigure}[9]{r}{0.5\linewidth}
\vspace{-10pt}
\includegraphics[width=\linewidth]{images/simclr+imputer_c.png}
\vspace{-10pt}
\caption{\textbf{\emph{Left}}: SimCLR. \textbf{\emph{Right}}: SimCLR adapted for ADIOS. }\label{fig:simclr+imputer}
\end{wrapfigure}


\paragraph{\acrshort{SSL} framework} 
%
\Cref{eq:imputer_siamese_obj} can be realised by simply optimising a Siamese network \citep{bromley1993siamese}.
%
However, this loss can be trivially minimised when all the representations for different inputs ``collapse'' to a constant.
%
This phenomenon is known as latent collapse, and has been addressed in many different ways in augmentation-based \acrshort{SSL}.
% where similar to \cref{eq:imputer_siamese_obj}, the goal is to minimise the distance between the representations of two augmented views of the same image.
%
% For instance, SimCLR \citep{chen2020simclr} utilises minibatch training, and repulses the representation of different images while attracting the same image's two augmented views; BYOL \citep{grill2020byol} prevents collapse by using a momentum encoder; SimSiam \citep{chen2021simsiam} does so by implementing a stop gradient operation for one of the Siamese network's forward pass.
%
% Notably, despite their differences, almost all augmentation-based \acrshort{SSL} methods optimise a loss that involves the term in \Cref{eq:imputer_siamese_obj}. 

Let us take SimCLR \citep{chen2020simclr} as an example (see \Cref{fig:simclr+imputer}, left); given a minibatch of $M$ input images $\x =\{\x_i\}_{i=1}^{M}$, two sets of random augmentations $A$ and $B$ are applied to each image in $\x$, yielding $\x^A$ and $\x^B$. 
%
The same encoding function $\I$ is used to extract representations from both sets of augmented views, yielding $\z^A=\I(\x^A)$ and $\z^B=\I(\x^B)$. 
%
The objective of SimCLR is defined as
%
\begin{align}
%\{\x^A_i, \x^B_i\}_{i=0}^N
    \mathcal{L}_{\text{SimCLR}}(\x; \I) =  \log \frac{\exp(\mathcal{D}(\z^A_i, \z^B_i))}{\sum_{i \neq j}\exp(\mathcal{D}(\z^A_i, \z^B_j))}, \label{eq:simclr_obj}
\end{align}
%
where $\mathcal{D}$ denotes the negative cosine similarity\footnote{Here we omit the temperature parameter in the original SimCLR loss for simplicity.}. 
%
Intuitively, the objective minimises the distance between representations of the two augmented views of the same image (i.e. $\z^A_i, \z^B_i$), while repulsing the representations of different images (i.e. $\z^A_i, \z^B_j$).
%
This effectively prevents the representations of different images from collapsing to the same constant, while optimising an objective similar to \Cref{eq:imputer_siamese_obj}.
% For instance, SimCLR \citep{chen2020simclr} utilises minibatch training, and repulses the representation of different images while attracting the same image's two augmented views; BYOL \citep{grill2020byol} prevents collapse by using a momentum encoder; SimSiam \citep{chen2021simsiam} does so by implementing a stop gradient operation for one of the Siamese network's forward pass.
%

W can use the SimCLR objective for our model by applying mask to one of the augmented image and then follow the exact same pipeline (see \Cref{fig:simclr+imputer}, right).
% 
More specifically, we replace $\z^A$ by $\z^{A,\m}=\I(\x^A\odot \m^A)$, where $\m^A = \M(\x^A)$ is a mask generated by the occlusion model given $\x^A$ as input.
%
Following \Cref{eq:simclr_obj}, we can write the SimCLR-ADIOS objective as
%
\begin{align}
%\{\x^A_i, \x^B_i\}_{i=0}^N
    & \mathcal{L}_{\text{SimCLR}}^{\text{ADIOS}}(\x; \I,  \M) = \log \frac{\exp(\mathcal{D}(\z^{A,\m}_i, \z^B_i))}{\sum_{i \neq j}\exp(\mathcal{D}(\z^{A,\m}_i, \z^B_j))}\notag \\ 
    &= \log \frac{\exp(\mathcal{D}(\I(\x^A_i\odot\M(\x^A_i)), \I(\x^B_i)))}{\sum_{i \neq j}\exp(\mathcal{D}(\I(\x^A_i\odot\M(\x^A_i)), \I(\x^B_j)))}.
    \label{eq:simclr_adios_obj}
\end{align}
%
Again, we can use $\mathcal{L}_{\text{SimCLR}}^{\text{ADIOS}}$ in \Cref{eq:minmax_obj} to train the inference-occlusion model.
%
Importantly, any \acrshort{SSL} method that compares the two augmented views of an image includes a term like \Cref{eq:imputer_siamese_obj} and can be plugged in to our framework.
%
We conducted experiments using the objective of SimCLR, BYOL \citep{grill2020byol} and SimSiam \citep{chen2021simsiam}, and show improvement on downstream task performance of each method significantly.

\subsection{Occlusion model $\M$}
%
For the sake of simplicity, we only considered the case where the occlusion model produces one mask only in the discussion above.
%
Since an image often contains multiple components, in practice, we generate $N>1$ masks to challenge the model to reason for different components, which we find in experiments is more beneficial for representation learning.

There are many parametric forms $\M$ could employ --- for instance, one could consider generating multiple masks sequentially in an auto-regressive manner as seen in \citet{engelcke2021genesis}.
%
However, here we find that the simplest solution suffice, where $\M: \RR^{c \times w \times h} \mapsto \RR^{N \times w \times h}$ consists of a learnable neural network and a softmax layer $\sigma$ applied across $N$ masks to ensure that all the masks sums to 1.
%
We have also experimented with binarising the masks during training, however we find that this does not improve results and therefore used real-valued masks directly.
%  and use a straight-through estimator for computing gradients\footnote{In PyTorch this can be implemented as \texttt{mask = binary\_mask + (mask - binary\_mask).detach()}.}



\subsection{Putting it together}

\begin{wrapfigure}[8]{r}{0.5\linewidth}
    \vspace{-15pt}
    \includegraphics[width=\linewidth]{images/model_ambiguous_k.png}
    \vspace{-10pt}
    \caption{ADIOS, $N>1$.} % The occluder first produce a mask $m$ from the image $x$, which is then applied to the image via element-wise product $x\cdotm$. The imputer extracts features $z$ and $\tilde{z}$ from the original image $x$ and the occluded image $x\cdotm$ respectively. The imputer and the occluder play a min-max game, where the imputer is trained to maximise the similarity between $z$ and $\tilde{z}$ and the occluder minimises it.}
    \label{fig:architecture_k}
\end{wrapfigure}

Here we present the final form of ADIOS incorporating the $N$-masks occlusion model.
%
The occlusion model first produces $N$ soft masks $\{\m^{(n)}\}_{n=1}^N$ from the RGB image $\x$. 
%
The inference model computes a loss $\mathcal{L}^{(n)}(\x;\I,\M)$ for each $\m^{(n)}$ and the final loss is computed by averaging across $N$ masks
%
% \begin{align}
%     \mathcal{L}_{\text{ADIOS}}(\x;\Theta, \Psi) = \frac{1}{N} \sum^N_{n=1} \mathcal{L}_n(\x;\I,\M).
% \end{align}
\begin{align}
    \I^\star, \M^\star = \arg\min_\I\max_\M  \frac{1}{N} \sum^N_{n=1} \mathcal{L}^{(n)}(\x; \I, \M). \label{eq:minmax_obj_n}
\end{align}
%

\paragraph{Sparsity penalty}
%
\begin{wrapfigure}[9]{r}{0.3\linewidth}
    \vspace{-15pt}
    \includegraphics[width=\linewidth]{images/penalty.png}
    \vspace{-15pt}
    \caption{Penalty.}
    \label{fig:penalty_plot}
\end{wrapfigure}
%
There exist a trivial solution for the min-max objective in \Cref{eq:minmax_obj_n} when $N>1$, where the occlusion model mask out an entire image using one slot only.
%
Specifically, amongst the $N$ masks generated by the masking model $\{\m^{(1)}, \m^{(2)}\cdots \m^{(N)}\}$, one mask $\m^{(n)}$ masks out the entire image with $\sum_h \sum_w \m^{(n)} = hw$, while no occlusion will be applied to the image for the rest of the masking slots $\{N\}_{\setminus n}$.

In order to avoid these degenerative solutions, we hope to introduce a term that discourages the occlusion model from generating all-one or all-zero masks.
%
Here, we make use of the inverse of the sine function (different from $\arcsin$) and propose the following sparsity penalty
%
\begin{align}
    p_n = \sin\left(\frac{\pi}{hw} \cdot \displaystyle \sum_{i=1}^h \sum_{j=1}^w \m_{ij}^{(n)} \right)^{-1}.
\end{align}
%
Importantly, $p_n$ goes to infinity as $\m^{(n)}$ approaches all-one or all-zero.
%
See \Cref{fig:penalty_plot} for a visualisation.
%
Minimising this penalty term with respect to $\M$ encourage the occlusion model to generate semantically meaningful mask and avoid the trivial solution of occluding the whole image or none at all. 

\paragraph{Final objective} We can now write our final objective as
%
\begin{align}
    \I^\star, \M^\star = \arg\min_\I\max_\M  \frac{1}{N} \sum^N_{n=1} \left( \mathcal{L}^{(n)}(\x; \I, \M) - \lambda p_n \right), \label{eq:final}
\end{align}
%
where $\lambda$ denotes the scaling for the penalty term.
%
% We conducted experiments using 3 different from of SSL objectives for $\mathcal{L}_n$, including 1) SimCLR as seen in \Cref{eq:simclr_adios_obj}, 2) SimSiam and 3) BYOL.
%
We also include the pseudocode of ADIOS in \Cref{sec:app_adios_pseudocode}.

==> 2methodsv3.tex <==
\section{Methodology}\label{sec:methods}

\paragraph{Set up}%
ADIOS consists of two components, inference model $\I$ and occlusion model $\M$ (see \Cref{fig:architecture}). 
%
Given an RGB image $\x$, the occlusion model produces an image-sized mask $\m=\M(\x)$ with values in $[0, 1]$.
% , where $\m \in \{0, 1\}^{h \times w}$ and $\x \in \RR^{c \times h \times w}$
% 
Inference model $\I$ takes original image $\x$ and an occluded image $\x^{\m} = \x\odot \m$
($\odot$ is the Hadamard product) as inputs, producing some output $\I(\x^m,\x)$, which is used
to compute the objective $\mathcal{L}$.
%
The models are learnt by solving the following min-max problem
%
\begin{align}
    \I^\star, \M^\star = \arg\min_\I\max_\M \mathcal{L}(\x; \I, \M)\,. \label{eq:minmax_obj} 
\end{align}
%
We will now introduce each component in detail.

\subsection{Inference model $\I$}
% 
\begin{wrapfigure}[6]{r}{0.45\linewidth}
    \vspace*{-4em}
    \includegraphics[width=\linewidth]{images/model_ambiguous.png}
    \vspace{-2em}
    \caption{\!\adios\ Architecture} % The occluder first produce a mask $m$ from the image $x$, which is then applied to the image via element-wise product $x\cdotm$. The imputer extracts features $z$ and $\tilde{z}$ from the original image $x$ and the occluded image $x\cdotm$ respectively. The imputer and the occluder play a min-max game, where the imputer is trained to maximise the similarity between $z$ and $\tilde{z}$ and the occluder minimises it.}
    \label{fig:architecture}
\end{wrapfigure}
%
% The role of the inference model is to produce a representation of the input.
% As discussed in \Cref{sec:intro}, the distance between the representations of the original and that of a masked image should be minimized.
% 
As discussed in \Cref{sec:intro}, the inference model should minimise some distance between the original and masked images.
%
Here, we discuss potential forms of this objective, arriving at our final framework using augmentation-based \gls{SSL} methods.
%
\paragraph{Distance in pixel space} \label{sec:ae_imputer}
%
One option would be to inpaint the masked image with the inference model, and train $\I$ by minimising the distance between the inpainted image and the original image in pixel space.
%
More specifically, we can define $\I$ as an auto-encoder consisting of encoder $q$ and decoder $p$, where $\I = p \circ q$. 
%
The model can be trained using the following reconstruction loss
%
\begin{align}
  \mathcal{L}_{\text{AE}}(\x; \I, \M)
  \!=\! \mathcal{D}(\x, p \circ q (\x^{\m}))
  \!=\! \mathcal{D}(\x, \I (\x\odot \M(\x))), \label{eq:imputer_ae_obj}
\end{align}
% = 
where $\mathcal{D}$ denotes some distance metric defined in pixel space.
%
Minimising \cref{eq:imputer_ae_obj} encourages the auto-encoder to impute the missing part of the image as accurately as possible. 
%
$\mathcal{L}_{\text{AE}}$ can then be used in \cref{eq:minmax_obj} to train the inference-occlusion model.

\paragraph{Distance in representation space}
%
An interesting question for auto-encoding $\I$ is: where does the imputation happen? 
%
Multiple hypotheses exist: 
%
\circled{1} \emph{\textbf{Encoder only:}} The encoder $q$ completely recovers the missing
information in the masked image, and in the ideal case, $q(\M(\x)) = q(\x)$; the decoder
faithfully reconstructs these representations.
%
\circled{2} \emph{\textbf{Decoder only:}} The encoder faithfully extracts all information from the masked image, and the decoder reasons to inpaint missing pixel from the representations;
%
\circled{3} \emph{\textbf{Both:}} The encoder and decoder both inpaint parts of the image.

Given these scenarios, \circled{1} is clearly best suited for representation learning, as it requires the encoder to reason about the missing parts based on observed context, beyond just extracting image features.
%
With representation learning, rather than inpainting, being our end goal, the key challenge lies
in designing an objective targetting scenario \circled{1}, such that we learn the most expressive version of encoder $q$.

A key feature in \circled{1} is that when the encoder recovers all information of the original image, $q(\x^{\m}) = q(\x)$, the features extracted from the partially observed image $\x^{\m}$ should in principle be the same as those extracted from the unmasked image $\x$.
%
We thus propose an encoding inference model $\I$ consisting of only the encoder, which extracts representation $\z =\I(\x)$, where $\z\in\RR^d$.
%
Our objective can therefore be written as 
%
\begin{align}
  \hspace*{-10pt}\mathcal{L}_{\text{ENC}}(\x;\I,\M)
  \!=\!\mathcal{D}(\z,\z^{\m}) % \notag \\
  \!=\! \mathcal{D}(\I(\x), \I(\x\!\odot\! \M(\x)))
  \hspace*{-5pt}\label{eq:imputer_siamese_obj}
\end{align}
%
where $\mathcal{D}$ is some distance metric defined in $\RR^d$.
%
Not only does $\loss_{\text{ENC}}$ encourages the learning of more expressive encoder that can infer missing information, optimising this objective also does not involve generative component $p$, which is redundant for representation learning.


\begin{wrapfigure}[8]{r}{0.55\linewidth}
  \vspace{-1.5\baselineskip}
  \includegraphics[width=\linewidth]{images/simclr+imputer_c.png}
  \vspace{-1.5\baselineskip}
  \caption{\textbf{\emph{Left}}:~SimCLR. \textbf{\emph{Right}}: SimCLR + ADIOS.}
  \label{fig:simclr+imputer}
\end{wrapfigure}
%
\paragraph{\acrshort{SSL} framework} 
%
\cref{eq:imputer_siamese_obj} can be realised by simply optimising a Siamese network \citep{bromley1993siamese}.
%
However, the objective can be trivially minimised when the representations for all inputs ``collapse'' to a constant.
%
This phenomenon, known as latent collapse, has been addressed in many ways in augmentation-based \acrshort{SSL}.
% where similar to \cref{eq:imputer_siamese_obj}, the goal is to minimise the distance between the representations of two augmented views of the same image.
%
% For instance, SimCLR \citep{chen2020simclr} utilises minibatch training, and repulses the representation of different images while attracting the same image's two augmented views; BYOL \citep{grill2020byol} prevents collapse by using a momentum encoder; SimSiam \citep{chen2021simsiam} does so by implementing a stop gradient operation for one of the Siamese network's forward pass.
%
% Notably, despite their differences, almost all augmentation-based \acrshort{SSL} methods optimise a loss that involves the term in \Cref{eq:imputer_siamese_obj}. 

Let us take SimCLR \citep{chen2020simclr} as an example (see \Cref{fig:simclr+imputer}, left); given a minibatch of $M$ input images $\x =\{\x_i\}_{i=1}^{M}$, two sets of random augmentations $A$ and $B$ are applied to each image in $\x$, yielding $\x^A$ and $\x^B$. 
%
The same encoding function $\I$ is used to extract representations from both sets of augmented views, yielding $\z^A=\I(\x^A)$ and $\z^B=\I(\x^B)$. 
%
The objective of SimCLR is defined as
%
\begin{align}
  % \{\x^A_i, \x^B_i\}_{i=0}^N
    \mathcal{L}_{\text{SimCLR}}(\x; \I) =  \log \frac{\exp(\mathcal{D}(\z^A_i, \z^B_i))}{\sum_{i \neq j}\exp(\mathcal{D}(\z^A_i, \z^B_j))}\,, \label{eq:simclr_obj}
\end{align}
%
where $\mathcal{D}$ denotes the negative cosine similarity\footnote{We omit the SimCLR temperature parameter for simplicity.}. 
%
Intuitively, the objective minimises the distance between representations of the two augmented views of the same image (i.e. $\z^A_i, \z^B_i$), while repulsing the representations of different images (i.e. $\z^A_i, \z^B_j$).
%
This effectively prevents the representations of different images from collapsing to the same constant, while optimising an objective similar to \Cref{eq:imputer_siamese_obj}.
% For instance, SimCLR \citep{chen2020simclr} utilises minibatch training, and repulses the representation of different images while attracting the same image's two augmented views; BYOL \citep{grill2020byol} prevents collapse by using a momentum encoder; SimSiam \citep{chen2021simsiam} does so by implementing a stop gradient operation for one of the Siamese network's forward pass.
%

We can use the SimCLR objective for our model by masking one of the augmented images and then follow the exact same pipeline (see \Cref{fig:simclr+imputer}, right).
% 
More specifically, we replace $\z^A$ by $\z^{A,\m}=\I(\x^A\odot \m^A)$, where $\m^A = \M(\x^A)$ is a mask generated by the occlusion model given $\x^A$.
%
Following \Cref{eq:simclr_obj}, we can write the SimCLR-ADIOS objective as
%
\begin{align}
  &\mathcal{L}_{\text{SimCLR}}^{\text{ADIOS}}(\x; \I,  \M)
    = \log \frac{\exp(\mathcal{D}(\z^{A,\m}_i, \z^B_i))}{\sum_{i \neq j}\exp(\mathcal{D}(\z^{A,\m}_i, \z^B_j))} \notag \\ 
  &= \log \frac{\exp(\mathcal{D}(\I(\x^A_i\odot\M(\x^A_i)), \I(\x^B_i)))}{\sum_{i \neq j}\exp(\mathcal{D}(\I(\x^A_i\odot\M(\x^A_i)), \I(\x^B_j)))}\,.
    \label{eq:simclr_adios_obj}
\end{align}
%
Again, we can use \cref{eq:simclr_adios_obj} in \Cref{eq:minmax_obj} to train the inference-occlusion model.
%
Crucially, any \acrshort{SSL} method that compares two augmented image views includes a term like \Cref{eq:imputer_siamese_obj}, and can be plugged in to our framework.
%
We conduct experiments using SimCLR, BYOL \cite{grill2020byol}, and SimSiam \cite{chen2021simsiam} objectives and show significant improvement on downstream task performance with each method.
%
Refer to \Cref{sec:app_objectives} for the ADIOS objective used for BYOL and SimSiam, as well as more details on the SimCLR objective.

\subsection{Occlusion model $\M$}
%
For simplicity, we only consider the single-mask-generating case in the discussion above.
%
In practice, since an image typically contains multiple components, we generate $N>1$ masks to challenge the model to reason about relations between different components---empirical performance confirm benefits of doing so.

There are many parametric forms $\M$ could employ.
%
For instance, one could consider generating multiple masks sequentially in an auto-regressive manner as seen in \citet{engelcke2021genesis}.
%
However, we find that the simplest setup suffices, where $\M: \RR^{c \times w \times h} \mapsto \RR^{N \times w \times h}$ consists of a learnable neural network and a pixelwise softmax layer $\sigma$ applied across $N$ masks to ensure that the sum of a given pixel across all the masks equals 1.
%
We use U-Net as the backbone of our occlusion model---see \Cref{sec:app_mask_arch} for more details.
%
Note that we experimented with binarising the masks during training, but found that this did not yield improvements, and hence used real-valued masks directly.
%

\subsection{Putting it together}

\begin{wrapfigure}[6]{r}{0.53\linewidth}
  \vspace{-3\baselineskip}
  \includegraphics[width=\linewidth]{images/model_ambiguous_k.png}
  \vspace{-20pt}
  \caption{ADIOS, $N>1$.} % The occluder first produce a mask $m$ from the image $x$, which is then applied to the image via element-wise product $x\cdotm$. The imputer extracts features $z$ and $\tilde{z}$ from the original image $x$ and the occluded image $x\cdotm$ respectively. The imputer and the occluder play a min-max game, where the imputer is trained to maximise the similarity between $z$ and $\tilde{z}$ and the occluder minimises it.}
  \label{fig:architecture_k}
\end{wrapfigure}

Here we present \adios\ in its complete form.
%
This includes the $N$-mask occlusion model, which generates masks $\{\m^{(n)}\}_{n=1}^N$ from the RGB image $\x$. 
%
The inference model computes a loss $\mathcal{L}^{(n)}(\x;\I,\M)$ for each $\m^{(n)}$ and the final loss is computed by averaging across $N$ masks
%
% \begin{align}
%     \mathcal{L}_{\text{ADIOS}}(\x;\Theta, \Psi) = \frac{1}{N} \sum^N_{n=1} \mathcal{L}_n(\x;\I,\M).
% \end{align}
\begin{align}
    \I^\star, \M^\star = \arg\min_\I\max_\M  \frac{1}{N} \sum^N_{n=1} \mathcal{L}^{(n)}(\x; \I, \M)\,. \label{eq:minmax_obj_n}
\end{align}

\begin{wrapfigure}[8]{r}{0.32\linewidth}
  \centering
  \vspace*{-2\baselineskip}
  \hspace*{-2ex}
  \includegraphics[width=0.92\linewidth]{images/penalty.png}
  \vspace{-0.8\baselineskip}
  \caption{Penalty.}
  \label{fig:penalty_plot}
\end{wrapfigure}
%
\paragraph{Sparsity penalty}
%
A trivial solution exists for this objective \Cref{eq:minmax_obj_n}, where, for masks $\{\m^{(1)}, \ldots, \m^{(N)}\}$, some mask $\m^{(n)}$ occludes everything, with the other \scalebox{0.98}{$\{N\}_{\setminus n}$} masks not occluding anything. % , $\sum_h \!\sum_w \!\m^{(n)} \!=\! hw$
%
To avoid such degenerate solutions, we introduce a sparsity penalty $p_n$ in the form of $\nicefrac{1}{sin(\cdot)}$ that discourages the occlusion model from generating all-one or all-zero masks; specifically,
\begin{align}
    p_n = \sin\left(\frac{\pi}{hw}\displaystyle \sum_{i=1}^h \sum_{j=1}^w \m_{ij}^{(n)} \right)^{-1}\,.
\end{align}
%
Note that, $p_n$ goes to infinity as $\m^{(n)}$ approaches all-one or all-zero (see \Cref{fig:penalty_plot}).
%
Minimising $p_n$ with respect to $\M$ encourages the occlusion model to generate semantically meaningful mask, while avoiding degenerate solutions.

\paragraph{Final objective} Let $\lambda$ the scaling of the penalty term. Our complete objective reads as
%
\begin{align}
    \I^\star, \M^\star = \arg\min_\I\max_\M  \frac{1}{N} \sum^N_{n=1} \left( \mathcal{L}^{(n)}(\x; \I, \M) - \lambda p_n \right)\,. \label{eq:final}
\end{align}
%
% We conducted experiments using 3 different from of SSL objectives for $\mathcal{L}_n$, including 1) SimCLR as seen in \Cref{eq:simclr_adios_obj}, 2) SimSiam and 3) BYOL.
%
% We include the complete pseudocode for \adios\ in \Cref{sec:app_adios_pseudocode}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

% LocalWords:  inpaint inpainted inpainting SimCLR minibatch BYOL SimSiam softmax binarising
% LocalWords:  pixelwise

